Privacy-Preserving Redaction of Diagnosis Data through Source Code Analysis

Protecting sensitive information in diagnostic data such as logs, is a critical concern in the industrial software diagnosis and debugging process. While there are many tools developed to automatically redact the logs for identifying and removing sensitive information, they have severe limitations which can cause either over redaction and loss of critical diagnostic information (false positives), or disclosure of sensitive information (false negatives), or both. To address the problem, in this paper, we argue for a source code analysis approach for log redaction. To identify a log message containing sensitive information, our method locates the corresponding log statement in the source code with logger code augmentation, and checks if the log statement outputs data from sensitive sources by using the data flow graph built from the source code. Appropriate redaction rules are further applied depending on the sensitiveness of the data sources to preserve the privacy information in the logs. We conducted experimental evaluation and comparison with other popular baselines. The results demonstrate that our approach can significantly improve the detection precision of the sensitive information and reduce both false positives and negatives.

==> background.tex <==
\section{Background}\label{sec:background}


==> relatedwork.tex <==
\section{Related Works}\label{sec:relatedwork}


Various privacy-preserving mechanisms are proposed for sharing data that contains sensitive information. These approaches strike different trade-offs among accuracy, privacy, efficiency, and usability. 
CryptDB~\cite{popa2011cryptdb} stores data on remote servers using homomorphic encryption. SMCQL~\cite{bater2017smcql} applies secure multi-party computation over private data federation. These approaches are expensive and introduce significant overheads. Data anonymization~\cite{ghinita2007fast}, K-anonymity \cite{sweeney2002achieving}, L-Diversity  \cite{machanavajjhala2007diversity}, Hybrid-k anonymity \cite{nergiz2014hybrid}, etc., suffer from re-identification attacks~\cite{narayanan2006break, pandurangan2014taxis} and they also lead to information loss.  In addition, the aforementioned techniques are mostly applicable to structured data that are managed in database systems.

Differential privacy~\cite{ding2017collecting, duchi2013local} becomes a promising approach because it can provide a formal guarantee of the privacy. However, it is challenging to apply differential privacy to perturb diagnostic data to strike a good trade-off between protection and data usability.


There are existing works in the detection and redaction of sensitive and/or personal information (e.g., enterprise customer information or project personnel information) in order to prepare data for sharing \cite{cumby2011machine}.%
Particularly, a number of rule-based tools, such as Google Cloud Data Loss Protection (DLP)~\cite{google-dlp}, Amazon Macie~\cite{amazon-macie}, Microsoft Presidio~\cite{microsoft-presidio}, have been developed to detect and redact the sensitive information from the diagnostics data based on pattern matching. However, as we pointed out earlier, these tools will suffer from the over-redacting issue. We observed that numerous non-sensitive messages, which are useful for diagnostics purposes, are redacted by mistake. 
In recent years, machine learning based log redaction approach \cite{he2020loghub} attracts community attention.%
However, such approaches requires significant overheads in labeling the ocean-volume log data for training models from scratch or for finetuning pre-trained language models, which is a laborious and time-consuming process. While in our approach, only the sensitive attributes of the structured data sources that are accessed by the software to be diagnosed (i.e., the producer of the diagnosis data) need to be labeled, which is significantly easier. %

